iWinRNFL: A Simple, Interpretable & Well-Calibrated In-Game Win Probability Model for NFL

During the last few sports seasons a lot of discussion has been generated for the several, high-profile, "comebacks" that were observed in almost all sports. The Cavaliers won the championship after being down 3-1 in the 2016 NBA finals' series against the Golden State Warriors, which was exactly the case for Chicago Cubs and the World Series. The Patriots won the Super Bowl in 2016 even though they were trailing by 25 points late in the third quarter, while FC Barcelona in the top-16 round of the 2016-17 Champions League scored 3 goals during the last 7 minutes of the game (including stoppage time) against PSG to advance in the tournament. This has brought the robustness and accuracy of the various probabilistic prediction models under high scrutiny. Many of these models are proprietary, which makes it hard to evaluate. In this paper, we build a simple and open, yet robust and well-calibrated, in-game probability model for predicting the winner in an NFL (iWinRNFL) game. In particular, we build a logistic regression model that utilizes a set of 10 variables to predict the running win probability for the home team. We train our model using detailed play-by-play data from the last 7 NFL seasons obtained through the league's API. Our results indicate that in 75% of the cases iWinRNFL provides an accurate winner projection, as compared to a 63% accuracy of a baseline pre-game win probability model. Most importantly the probabilities that iWinRNFL provides are well-calibrated. Finally, we have also evaluated more complex, non-linear, models using the same set of features, without any significant improvement in performance.

==> Untitled.tex <==
\section{Introduction}
\label{sec:intro}

In-game win probability models provide the likelihood that a certain team will win a game given the current state of the game.  
Such models have become very popular during the last few years, mainly because they can provide the backbone for in-game decisions but also because they can potentially add to the viewing experience of the fans.

==> background.tex <==
\section{Background}
\label{sec:background}

Predicting the outcome of a sports game - and in particular American football in our case - has been of interest for several decades now. 
For example, Stern \cite{stern91} used data from the 1981, 1983 and 1984 NFL seasons and found that the distribution of the win margin follows a normal distribution with mean equal to the pregame point spread and standard deviation a little less than 14 points.  
He then used this observation to estimate the probability distribution of the number of games won by a team.  
The most influential work in the space, Win Probability Added, has been developed by Burke \cite{wpa} who uses various variables such as field position, down etc. to predict the win probability added after every play.  
This work forms the basis for ESPN's prediction engine, which uses an ensemble of machine learning models.   
Inspired by the early work and observations from Stern Winston developed an in-game win-probability model \cite{winston2012mathletics}, which was further adjusted from Pro-Football Reference to form their P-F-R win probability model using the notion of expected points \cite{pfrmodel}.  
More recently, Lock and Nettleton \cite{lock2014using} provided a random forest model for in-game win probability, while Shneider \cite{gambletron} created a system that uses real-time data from betting markets to estimate win probabilities. 
Finally, similar in-game win probability models exist for other sports (e.g., \cite{buttrey2011estimating,stern1994brownian}). 

One of the main reasons we introduce {\method} despite the presence of several in-game win probability models is the fact that the majority of them are hard to reproduce either because they are proprietary or because they are not described in great detail.  
Furthermore an older model, might not be applicable anymore ``as-is'' given the changes the game undergoes over the years (e.g., offenses rely much more on the passing game today as compared to a decade ago). 
Our goal with this work is twofold; (i) to provide an {\em open}\footnote{Source code and data will be made publicly available.}, simple, yet well-calibrated, in-game win probability model for the NFL, and (ii) to emphasize on the appropriate ways to evaluate such models. 
%The latter has been largely ignored in the current literature.  

==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, motivated by several recent comebacks that seemed improbable at the moment, we designed {\method}, a simple generalized linear model for in-game win probabilities in NFL. 
{\method} uses 10 independent variables to assess the win probability of a team for any given state of the game. 
Our evaluations indicate that the probabilities provided by our model are consistent and well-calibrated. 
One crucial point is that the developed models need to be re-evaluated frequently.  
The game changes rapidly both due to changes in the rules but also because of changes in players skills or even due to analytics (e.g., see the explosion of three-point shots in basketball, or the number of NFL teams that are now run a pass-first offense).  
Hence, the details of the model can also change due to these changes.  

Finally, win probability models, while currently are mainly used from media in order to enhance sports storytelling, can form a central component for the evaluation of NFL players. 
In particular, the added win probability from each player can form the dependent variable in a (adjusted) plus-minus type of regression. 
In the future we plan to explore similar applications of {\method} related with personnel decision, in-game adjustments etc.

==> evaluation.tex <==
\section{Model Evaluation}
\label{sec:evaluation}

We begin by evaluating how well the output probabilities of {\method} follow what happens in reality.  
When a team is given a 70\% probability of winning at a given state of the game, this essentially means that if the game was played from that state onwards 100 times, the team is expected to win approximately 70 of them.  
Of course, it is clear that we cannot have the game played more than once so one way to evaluate the probabilities of our model is to consider all the instances where the model provided a probability for team winning $x\%$ and calculate the fraction of instances that ended up in a win for this team.  
Ideally we would expect this fraction to be $x\%$ as well. 

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.25]{plots/fullwinprob.pdf}%\vspacecap
 \caption{{\method} is consistent over the whole range of probabilities.}
 \label{fig:fullwp}
\end{center}
\end{figure}

In order to obtain these results we split our data in a training and test set in a 70-30\% proportion respectively.    
Figure \ref{fig:fullwp} presents the results on our test set, where we used bins of a 0.05 probability range. 
In particular, as we can see the predicted probabilities match very well with the actual outcome of these instances.  
The fitted line has a slope of 1.007 (with a 95\% confidence interval of [0.994,1.019]), while the intercept is -0.005 (with a 95\% confidence interval [-0.013, 0.0014]), while the $R^2 = 0.99$.  
Simply put the line is for all practical purposes the $y=x$ line, which translates to a fairly consistent and accurate win probability. 

We have also calculated the accuracy of our binary predictions (i.e., without loss of generality the home team is projected to win if $\Pr(H=1| \mathbf{x})>0.5$) on the test set and is equal with 74\%, that is, our predictions are correct in 74\% of the instances.  
Another metric that has been traditionally used in the literature to evaluate the performance of a probabilistic prediction is the Brier score $\brier$ \cite{brier1950verification}.  
In the case of a binary probabilistic prediction the Brier score is calculated as: 

\begin{equation}
\brier = \dfrac{1}{N}\sum_{i=1}^N (\pi_i-y_i)^2
\label{eq:brier}
\end{equation}
where $N$ is the number of observations, $\pi_i$ is the probability assigned to instance $i$ being equal to 1 and $y_i$ is the actual (binary) value of instance $i$.  
Brier scores takes values between 0 and 1 and does not evaluate the accuracy of the predicted probabilities but rather the calibration of these probabilities, that is, the level of certainty they provide.  % (e.g., a 0.9 probability is more calibrated compared to a 0.55 probability).   
The lower the value of $\brier$ the better the model performs in terms of calibrated predictions. 
Our model exhibits a Brier score $\brier$ of 0.17.  
Typically the Brier score of a model is compared to a baseline value $\brier_{base}$ obtained from a {\em climatology} model \cite{mason2004using}. 
A climatology model assigns the same probability to every observation (that is, home team win in our case), which is equal to the fraction of positive labels in the whole dataset.  
Hence, in our case the climatology model assigns a probability of 0.57 to each observation, since 57\% of the instances in the dataset resulted to a home team win. 
The Brier score for this reference model is $\brier_{base}=0.26$, which is obviously of lower quality as compared to our model. 

Next we examine the performance of {\method} as a function of the time elapsed from the beginning of the game, and in particular we consider the quarter of the predicted instance.  
Table \ref{tab:results} presents the results for the accuracy, the Brier score as well as the probability accuracy of {\method}. 
The latter is reflected on the 95\% confidence interval of the slope and intercept of the corresponding line (see Figure \ref{fig:fullwp}). 
As we can see the performance of {\method} improves as the game progresses. 
For example, during the first quarter the accuracy with which the winner is predicted is close to the state-of-the-art prediction accuracy of pre-game win probability models \cite{kpele-plosone}. 
However, as the game progresses {\method} is able to adjust its predictions. 

\begin{table*}
\centering
\begin{tabular}{c||*{2}{c|}c|c}
 & \multicolumn{2}{|c|}{Probability line} & & \\ \hline \hline
Quarter & Slope & Intercept & Brier score & Accuracy \\ \hline
1 & [0.87,0.95] & [0.041,0.088] & 0.21 & 0.64 \\ \hline
2 & [0.89,0.97] & [0.035,0.071] & 0.18 & 0.71 \\ \hline
3 & [0.97,1.03] & [-0.01,0.05] & 0.14 & 0.77 \\ \hline
4 & [0.99,1.21] & [-0.11,0.04] & 0.11 & 0.84 \\ \hline
\end{tabular}
\caption{The performance of our model improves as the game progresses.}
\label{tab:results}
\end{table*}

\iffalse
Qtr1 --> Intercept: 0.01724886 0.08667382 Slope: 0.85147882 0.97192799 Brier: 0.21 (0.25)
Qtr2 --> Intercept: 0.03572466 0.09115063 Slope: 0.84114141 0.93719396 Brier: 0.18 (0.25)
Qtr3 --> Intercept: -0.01549244 0.05285255 Slope: 0.91602858 1.03443241 Brier: 0.14 (0.25)
Qtr4 --> Intercept: -0.1120115 -0.0448949 Slope:  0.9970946  1.2132215 Brier: 0.11 (0.25)
Accuracy --> 0.64 0.71 0.77 0.84
\fi

{\bf Anecdote {\em Evaluation}: }
As mentioned in the introduction, one of the motivating events for {\method} has been Super Bowl 51. 
Super Bowl 51 has been labeled as the biggest comeback in the history of Super Bowl.  
Late in the third quarter New England Patriots were trailing by 25 points and Pro Football Reference was giving Patriots a 1:1000 chance of winning the Super Bowl, while ESPN a 1:500 chance \cite{statsbylopez}. 
PFR considers this comeback a once in a millennium comeback. 
While this can still be the case\footnote{As mentioned earlier 1:$x$ chances does not mean that we observe $x$ {\em failures} first and then the one {\em success}.}, in retrospect Patriots' win highlights that these models might be too optimistic and confident to the team ahead.  
On the contrary, the lowest probability during the game assigned to the Patriots by {\method} for winning the Super Bowl was 2.1\% or about 1:50.  %, i.e., once every half century, which seems more reasonable.  
We would like to emphasize here that the above does not mean that {\method} is ``{\em better}'' than other win probability models.  
However, it is a simple, open model that assigns win probabilities in a conservative (i.e., avoids ``over-reacting''), yet accurate and well-calibrated way.  


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.4]{plots/sb51.png}%\vspacecap
 \caption{The lowest in-game win probability assigned to the Patriots by {\method} during Super Bowl 51 was 2.1\%, i.e., 1 in 50 chances. During the OT the model does not perform very accurately due to the sparsity of the relevant data.}
 \label{fig:sb51}
\end{center}
\end{figure}

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

In-game win probability models provide the likelihood that a certain team will win a game given the current state of the game.  
Such models have become very popular during the last few years, mainly because they can provide the backbone for in-game decisions but also because they can potentially improve the viewing experience of the fans.  
Among other events this year's super bowl sparked a lot of discussion around the validity and accuracy of these models \cite{ringer17} since at some point late in the third quarter the probability given by some of these models to New England Patriots to win was less than 0.1\% or in other words a 1 in 1,000 Super Bowls comeback \cite{statsbylopez}.  
Clearly the result of the game was not the one projected at that point and hence, critiques of these models appeared.  

In this paper, we present the design of an in-game win probability model for NFL ({\method}) focusing on its appropriate evaluation.  
While {\method} is simple - at its core is based on a generalized linear model - our evaluations show that it is well-calibrated over the whole range of probabilities.  
Our model was trained using NFL play-by-play data for the past 8 seasons.  
The fact that New England Patriots won the Super Bowl even though they were given just 0.1\% probability to do so at the end of the third quarter, is not a {\em failure of the math}.  
In fact, this number tells us that roughly for every 1,000 times that a team is in the same position there will be 1 instance where the trailing team will win.  
Of course, the order with which we observe this instance is arbitrary - it can be the first time we ever observe this game setting (i.e., a team trailing with 25 points by the end of the third quarter) - which intensifies the opinion that {\em math failed}. 
So the real accuracy question is how well the predicted probabilities capture the actual winning chances of a team at a given point in the game.  
In other words, what fraction of the in-game instances where a team was given x\% probability of winning actually ended up with this team winning?  
Ideally, we would like this fraction to be also x\%, and we show that this is the case for {\method} over the whole range of probabilities. 

The rest of the paper is organized as follows: 
Section \ref{sec:background} briefly presents background on the win probability models for NFL.  
Section \ref{sec:model} presents our model, while Section \ref{sec:evaluation} presents the evaluation of {\method}.  
Finally, Section \ref{sec:conclusions} concludes our work and presents our future directions. 


==> method.tex <==
In this section we will introduce the network structure we use for our ranking scheme as well as our approach. 

\begin{lemma}[{\tt League Network} definition]
The league network $\net=(\nodes,\edges)$, is a weighted directed network where an edge $\edge_{i,j} \in \edges$ points from node $i\in \nodes$ to node $j\in \nodes$ iff team $j$ has won against team $i$.  The edge weight $\weight_{\edge_{i,j}}$ is equal to the point differential of the corresponding game.
\label{def:net}
\end{lemma}  

The league network $\net$ captures ``who-wins-against-whom'' and by what margin.  
With $\bm{\beta}$ being a vector whose $i$-th element captures external (i.e., irrelevant from the network structure) factors affecting the strength of team $i$ (e.g., total budget, number of pro-ball players in the roster, total offense, total defense etc.), the PageRank of $\net$ is given by: 

\begin{equation}
\bm{\pi} = D(D-\alpha A)^{-1}\bm{\beta}
\label{eq:pr}
\end{equation}

\noindent where $A$ is the adjacency matrix of $\net$, $\alpha$ is a parameter (a typical value of which is 0.85) and $D$ is a diagonal matrix where $d_{ii} = \max(1,k_{i,out})$, with $k_{i,out}$ being the out-degree of node $i$.  
While in most practical cases PageRank considers only the network structure, Eq. (\ref{eq:pr}) is able to take into consideration - if needed - not only the network structure but external information that affect the ``power'' of team $i$ through vector $\bm{\beta}$.  
Figure \ref{fig:net} depicts the network obtained using all the games from the last NFL regular season.  
The edge width is proportional to the score differential in the corresponding game, while the vertex size is proportional to the node's PageRank score. 

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.32,angle=270]{plots/net.pdf}%\vspacecap
 \caption{The directed NFL League Network for the regular season 2015-2016.  More ``powerful'' nodes are represented with larger vertex size.}
 \label{fig:net}
\end{center}
\vspace{-0.2in}
\end{figure}


The rationale behind using PageRank is that compared to simple team standings that capture the fraction of wins for a team, PageRank further indirectly considers the strength of the opponent. 
In other words, it does not only matter to win but also to win an important team in order to improve in the rankings.  
In what follows we evaluate and delve into the details of the performance of {\method}.

==> model.tex <==
\section{The \MakeLowercase{i}W\MakeLowercase{inr}NFL model}
\label{sec:model}

In this section we are going to present the data we used to develop our in-game probability model as well as the design details of {\method}. 

{\bf Data: }In order to perform our analysis we utilize a dataset collected from NFL's Game Center for all the regular season games between the seasons 2009 and 2016. 
We access the data using the Python {\tt nflgame} API \cite{nflgame}. 
The dataset includes detailed play-by-play information for every game that took place during these seasons. 
This information is used to obtain the state of the game that will drive the design of {\method}. 
In total, we collected information for 2,048 regular season games and a total of 338,294 snaps/plays. 

{\bf Model: }
{\method} is based on a logistic regression model that calculates the probability of the home team winning given the current status of the game as: 

\begin{equation}
\Pr(H=1| \mathbf{x})= \frac{\exp(\mathbf{\weight}^T\cdot\mathbf{x})}{1+\exp(\mathbf{\weight}^T\cdot\mathbf{x})}
\label{eq:reg}
\end{equation}
where $H$ is the dependent random variable of our model representing whether the home team wins or not, $\mathbf{x}$ is the vector with the independent variables, while the coefficient vector $\mathbf{\weight}$ includes the weights for each independent variable and is estimated using the corresponding data.  
For a game of infinite duration a linear model could be a very good approximation.  
However, the boundary effects from the finite duration of a game create several non-linearities \cite{winston2012mathletics}.  
For this reason, we enhance our model - using the same set of features - with a Support Vector Machine classifier with radial kernel for the last three minutes of regulation.  
In order to obtain a probability output from the SVM classifier, we further use Platt's scaling \cite{platt1999probabilistic}: 

\begin{equation}
\Pr(H=1| \mathbf{x})= \frac{1}{1+\exp{(Af(x)+B)}}
\label{eq:platt}
\end{equation}
where $f(x)$ is the uncalibrated value produced by the SVM classifier: 

\begin{equation}
f(x) = \sum_{i} (\alpha_i y_i k(\mathbf{x}_i\cdot\mathbf{x}))+ b
\label{eq:svm}
\end{equation}
where $k(\mathbf{x},\mathbf{x}')$ is the kernel used for the SVM.   
Figure \ref{fig:iwinrNFL} depicts the simple flow chart of {\method}. 


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.35]{plots/iwinrNFL.pdf}%\vspacecap
 \caption{{\method} includes a linear and a non-linear component.}
 \label{fig:iwinrNFL}
\end{center}
\end{figure}

In order to describe the status of the game we use the following variables:

\begin{enumerate}
\item {\bf Ball Possession Team:} This binary feature captures whether the home or the visiting team has the ball possession
\item {\bf Score Differential:} This feature captures the current score differential (home - visiting)
\item {\bf Timeouts Remaining:} This feature is represented by two independent variables - one for the home and one for the away team - and they capture the number of timeouts remaining for each of the teams
%\item {\bf Quarter:} This feature captures the current quarter of the game
%\item {\bf Time Remaining:} This feature captures the time (in seconds) remaining for the current quarter to end
\item {\bf Time Elapsed: } This feature captures the time elapsed since the beginning of the game
\item {\bf Down:} This feature represents the down of the team in possession
\item {\bf Field Position:} This feature captures the distance covered by the team in possession from their own yard line
\item {\bf Yards-to-go:} This variables represents the number of yards needed for a first down
\item {\bf Ball Possession Time: } This variable captures the time that the offensive unit of the home team is on the field 
\item {\bf Ranking Differential: } This variable represents the difference of the win percentage for the two team (home - visiting)
\end{enumerate}

The last independent variable is representative of the power ranking difference between the two teams. 
Most of the existing models that include such a variable are using the Vegas line spread for each game.  
We choose not to do so for the following reason.  
The objective of the Vegas line is not to predict game outcomes but rather distribute money across the different bets.  
Exactly because of this objective the line is changing during the week before the game.  
While this line can change due to new information for the competing teams (e.g., injury updates), the line is mainly changing when a particular team has accumulated the majority of the bets. 
In this case it will also be hard to choose which line to use (e.g., the opening, the closing or some average of them).  
Therefore, we choose to use the win percentage differential of the two teams as an indicator of their strength (even though this has its own issues given the uneven schedule in NFL).  
However, note that if one would like to use the point spread as a variable this can be easily incorporated in the model. 
Table \ref{tab:iwinrnfl} presents the coefficients of the logistic regression model of {\method} with standardized independent variables for better comparisons. 


\begin{table}[ht]
\begin{center}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{Winner}\\
\midrule
Possession Team (H)         &      0.41\sym{***}\\
                    &     (49.19)         \\
\addlinespace
Score Differential           &      3.59\sym{***}\\
                    &    (247.34)         \\
\addlinespace
Home Timeouts           &     0.12\sym{***}\\
                    &      (8.74)         \\
\addlinespace
Away Timeouts           &     -0.11\sym{***}\\
                    &    (-12.47)         \\
\addlinespace
Ball Possession Time  &     -0.05.\\
                    &    (-1.66)         \\
\addlinespace
Time Lapsed       &   -0.05.\\
                    &      (-1.66)         \\
\addlinespace
Down                &   -0.01         \\
                    &      (0.04)         \\
\addlinespace
Field Position            &   0.02\sym{**} \\
                    &      (2.71)         \\
\addlinespace
Yards-to-go                &  -0.01         \\
                    &      (0.23)         \\
\addlinespace
Rating differential         &       0.75\sym{***}\\
                    &     (80.47)         \\
\addlinespace
Intercept            &       0.57\sym{*}\\
                    &    (2.09)         \\
\midrule
Observations        &      338,294         \\
\bottomrule
\multicolumn{2}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{2}{l}{\footnotesize \sym{$_.$} \(p<0.1\), \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{center}
\caption{Standardized logisitic regression coefficients for {\method}.}
\label{tab:iwinrnfl}
\end{table}


As we can see, as one might have expected the current scoring differential exhibits the strongest correlation with the in-game win probability.  
The only factors that do not appear to be statistically significant predictors of the dependent variable are the down and the yards-to-go. 
Even though the corresponding coefficients are negative as one might have expected (e.g., being at an earlier down gives you more chances to advance the ball), they are not significant in estimating the win probability. 
On the contrary, all else being equal timeouts appear to be quiet important since they can help a team stop the clock, while teams with better win percentage appear to have an advantage as well, since this can be a sign of a better team. 
In the following section we provide a detailed evaluation of {\method}.

==> related.tex <==
Various approaches for ranking teams have appeared through the years.  
The simplest one - that is actually used in professional sports as the basis for advancing to playoffs - is the winning percentage, i.e., simply the fraction of games won by a team.  
Other ranking techniques consider the strength of the opponents and are based on the assumption that not all the wins are equal (e.g., \cite{rpi1}).  
One of the most well-known sports ranking methods is Elo ranking \cite{elo1978rating}, which assigns teams with an initial number of ``rating credits'' and based on the outcome of the games (compared to the expected one) these credits are exchanged between the teams.  
While the dominant network-based approach for ranking teams are based on PageRank, Park and Newman \cite{park2005network} proposed an interesting approach for cases where not every team plays against every other team in the league.  
They introduce the idea of ``indirect wins'', i.e., directed paths of length $k$, and apply a method that resembles Katz centrality to rank the teams.  
A comparison of various ranking systems can be found in \cite{barrow13,chartier11}, while a comprehensive list of the corresponding literature is compiled by Wilson \cite{wilson}.

At a tangential line of research hybrid voting-ranking systems, such as the Borda count and the Condorcet method \cite{stahl06}, have been utilized in the sports industry.  
Variations of these methods are used for handing the Heisman Trophy as well as the NBA's MVP. % Most Valuable Player.  
The Associated Press is also using a similar voting/ranking scheme to obtain the college teams ranking \cite{ap-ncaa}.  
Finally, probabilistic models for modeling the intransitivity in game data for predicting the outcome of match-up have also been recently proposed \cite{chen2016modeling,chen2016kdd}.

==> results.tex <==
In this section we evaluate {\method} through its ability to predict upcoming match-ups.  
In particular, let us assume that we want to predict the results of week $\tau$.  
Using the games up to that week, i.e., between week 1 and week $\tau-1$, we build the league network $\net_{\tau-1}$.  
This network will provide us with a ranking $\bm{\pi}(\tau-1)$. 
The prediction algorithm simply goes over this ranking and predicts as the winner of the match-up $i$-VS-$j$ team $i$, if $\pi_i(\tau-1) > \pi_j(\tau-1)$.  

Table \ref{tab:results} depicts the accuracy results obtain on the NFL dataset.  
We also present the accuracy of a similar baseline algorithm where the ranking is based on the winning percentage of the team.  
As we can see {\method} outperforms the baseline that uses simply the winning percentages.  
The overall accuracy of {\method} is 59\% with a standard error of 1.2\%, while that of the winning percentages is only 52\% with a standard error of 1.2\%.  
We would like to emphasize here that a 59\% accuracy is very close to the current state-of-the-art.  
In particular, during the last two years that Microsoft's Cortana \cite{cortana} is used to predict NFL game outcomes, the corresponding accuracy is not statistically significant different compared to the {\method}.  
More specifically for the season 2014-2015, Cortana exhibited a 66.4\% accuracy with a standard error of 2.9\% (compared with PageRank's 65.8\% with a standard error of 3\%), while for 2015-2016 Cortana's performance was 62.9\% with standard error 3\% (contrast with {\method}'s 59\% within 3\% standard error).  
Finally, the NFL league network is disconnected for the two first weeks of the season, and hence, {\method} can be confidently used for ranking teams after week 3.  
The results presented in Table \ref{tab:results} correspond to $\bm{\beta} = \bm{1}$.  
We have performed experiments where $\beta_i$ is set equal to the winning percentage of team $i$ and the results were indistinguishable.  

\begin{table}[ht!]
\centering
\begin{tabular}{c||c|c}
Year & {\method} & Winning Percentage\\
\hline
\hline
%05/30-05/31& 2& Art \& Craft Festival\\
% \hline
2009 & 0.64 & 0.57 \\ %0.033 \\ % 0.57 0.034
\hline
2010 & 0.56 & 0.5 \\ %0.034 \\ % 0.5 0.035
\hline 
2011 & 0.64 & 0.58 \\ %0.033\\  % 0.58 0.034
\hline
2012 & 0.65 & 0.56\\ %0.033 \\ % 0.56 0.035
\hline 
2013 & 0.56 & 0.5 \\ %0.034 \\ % 0.5 0.035
\hline
2014 & 0.66 & 0.56\\ %0.033 \\ % 0.56 0.034
\hline
2015 & 0.59 & 0.53 \\ %0.034\\ % 0.53 0.035
 \hline
\end{tabular}
\caption{Prediction accuracy with the {\method} is better as compared to that  of the simply winning percentages for each of the last 7 NFL seasons.}
\label{tab:results}
\end{table}

For the case of the NBA league network for the season 2014-15, {\method} provided an accuracy of 67\%, while the baseline method came close to it with a 66\% accuracy.  
Compared to the NFL case, NBA teams play many more games, and hence, despite a few ``surprising'' results, overall even the simple winning percentage provides a fairly good power ranking.  
In order to further explore this we compute the accuracy of {\method} and the baseline method in 4 different parts of the season.  
In particular, we divide the season into 4 parts, each of which covers approximately a 40-day period, and we calculate the corresponding accuracy.  
The results are presented in Figure \ref{fig:nba}.  
As we can see the performance gap is much larger during the beginning of the season, when the winning percentage of the teams has not converge to the real one.  
Later in the season the gap is reduced and the two methods provide essentially indistinguishable performance.  
With respect to the absolute performance, during the last quarter of the season the prediction accuracy is the highest, possibly due to the fact that the ranking (either through {\method} or through the winning percentage) has converged to one that reflects the actual power of the teams.  

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.35]{plots/nba.pdf}%\vspacecap
 \caption{Even though overall {\method} provides only marginal benefits over the winning percentage ranking, it is able to provide a good ranking early in the season.}
 \label{fig:nba}
\end{center}
\vspace{-0.2in}
\end{figure}

One of the problematic structures for PageRank are cycles in the network.  
In our case this corresponds to scenarios where team A has beaten team B, B has beaten team C and C has beaten team A. 
An acyclic network would provide a total order ranking, which in theory would have the highest accuracy.  
However, this is not the case in reality and cycles exists.  
Actually, given the fact that an NFL season consists of much fewer games than an NBA season (and not every teams plays with all the other teams), such cycles are expected to be less common.  
Hence, in what follows we examine the impact of the cycles on the performance of {\method}.  

In particular, we first calculate the minimum number of edges that one needs to remove from the network in order for it to be acyclic.  
This corresponds to the minimum feedback arc set problem \cite{eades1993fast}.  
Consequently, we compute the correlation between the fraction of edges in the minimum arc set and the difference in the performance between {\method} and the baseline approach.  
In particular, we compute the minimum arc set for the network after every game week for NFL and after every game day for NBA.  
Obtaining the correlation between the minimum arc set and the difference in the accuracy of {\method} and the baseline gives as {\bf -0.19 (p-value = 0.015) for NBA} and {\bf -0.21 (p-value = 0.039) for NFL}.  
The negative (and significant) correlation essentially means that {\method} is expected to outperform the winning percentage ranking as the network includes fewer directed cycles.  

Summarizing our results, we can say that {\method} is able to capture the interactions between teams better than the simple winning percentage ranking used in determining the teams that advance to the playoffs. 
In particular, in the case of NFL {\method} outperforms the baseline by approximately 7\%.  
In the case of NBA, the two approaches perform similar to each other, however, {\method} is able to converge to the appropriate ranking earlier in the season.  

% NBA -0.19 (0.01462)
% NFL -0.21 (0.03882)



==> table_res_vert.tex <==
\begin{tabular}{
@{\hspace{1ex}}l
@{\hspace{1.5ex}}c
@{\hspace{0.2ex}}c
@{\hspace{1.0ex}}c
@{\hspace{0.2ex}}c
@{\hspace{1.5ex}}c
@{\hspace{0.2ex}}c
@{\hspace{1.0ex}}c
@{\hspace{0.2ex}}c
@{\hspace{1ex}}}
%\toprule
 & & \multicolumn{2}{c}{\sumproblem} & & & \multicolumn{2}{c}{\minproblem} & \\
\cmidrule{2-4} \cmidrule{6-8}
 & & \datachic & \dataphily & & & \datachic & \dataphily & \\
\midrule
Total & & 2400~ & 2400~ & & & 2400~ & 2400~ & \\ [1ex]
$\abs{\solset}=1$ & & 111 & 407 & & & 263 & 562 & \\
$\abs{\solset}=2$ & & 182 & 148 & & & 317 & 253 & \\ [1ex]
Ident. \appfive & & 520 & 476 & & & 398 & 424 & \\
Ident. \appten & & 420 & 407 & & & 340 & 351 & \\
Ident. \apptwenty & & 337 & 327 & & & ~14 & ~49 & \\
%\bottomrule
\end{tabular}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> tensorrank.tex <==
The presence of cycles in the directed league network will always appear and cause problems, regardless of what method is used for ranking.  
However, it is possible to use additional information in order to break the ``gridlock'' in these situations.  
In particular, we propose to utilize tensor theory in order to account for multiple attributes simultaneously.  
More specifically, we have the following definition: 

\begin{lemma}[{\tt League Tensor} definition]
The league tensor $\tensor{T}(i,j,t)$, captures the temporal evolution of the win-loss relationships between the league teams. In particular, the entry $\tensor{T}(i,j,t)=\delta > 0$ if team $j$ won against team $i$ during game $t$ by $\delta$ points differential. 
\label{def:tens}
\end{lemma}  

One way to identify latent patterns in the data modeled by the tensor - which can then be used to rank entities in the dataset - is the PARAFAC decomposition \cite{parafac}.  
In particular, PARAFAC decomposes $\tensor{T}$ to a sum of $F$ components (see Figure \ref{fig:tensor}), such that: 
\begin{equation}
\tensor{T} \approx \displaystyle {\sum_{f=1}^F  \mathbf{a}_f \circ \mathbf{b}_f \circ \mathbf{c}_f },
\label{eq:tesor_dec}
\end{equation}
where $ \mathbf{a}_f \circ \mathbf{b}_f \circ \mathbf{c}_f (i,j,k) = \mathbf{a}_f(i) \mathbf{b}_f (j) \mathbf{c}_f (k) $. 
In other words, each component, i.e., triplet of vectors, of the decomposition is a rank one tensor.
Each vector in the triplet corresponds to one of the three modes of the tensor: $\mathbf{a}$ corresponds to the losing teams, $\mathbf{b}$ corresponds to the winning teams, and $\mathbf{c}$ corresponds to the time (game week/day).
Each of these $F$ components can be considered as a cluster, and the corresponding vector elements as soft clustering coefficients. 
We can then process the components that correspond to the teams (i.e., $\mathbf{a}$ and $\mathbf{b}$) in order to obtain a final ranking of the teams.   
%For notational simplicity, we denote as matrix $\mathbf{A}$ (and matrices $\mathbf{B}$ and $\mathbf{C}$ accordingly) the factor matrix that contains the $\mathbf{a}_f$ vectors as columns.
%Note that for the purposes of this work, we use the, highly optimized, Tensor Toolbox for Matlab \cite{tensortoolbox}.

\begin{figure}[t]
\begin{center}
\vspace{-0.35in}
\includegraphics[scale=0.25,angle=270]{plots/tensor.pdf}%\vspacecap
\vspace{-0.4in}
 \caption{The PARAFAC decomposition of the league tensor can capture latent patterns in the win-lose interactions of the teams that can facilitate power ranking.}
 \label{fig:tensor}
\end{center}
\vspace{-0.2in}
\end{figure}

The above decomposition is the central building block of {\methodt}.  
We can further enhance the ranking by utilizing non-network elements for the teams. 
In particular, every team is associated with a variety of performance indices (e.g., for the case of NFL these can include offensive/defensing yards per game, turnovers per game etc.).  
This information can be represented by a matrix $\bm{Y}$, where each row corresponds to a team and the columns correspond to the external attributes.  
Matrix $\bf{Y}$ is said to be coupled with league tensor $\tensor{T}$ at the team dimension, since they share this dimension in common.  
If we want to differentiate the performance of a team during the wins and the loses, we can create two matrices $\bm{Y}_w$ and $\bm{Y}_l$ that correspond to the performance metrics of the teams only during the winning and losing games respectively.  
Both of these matrices are coupled with the league tensor ($\bm{Y}_w$ is coupled with the winning team dimension while $\bm{Y}_l$ is coupled with the losing team dimension). 
%
In general an $n$-dimensional tensor can be coupled with at most $n$ matrices $\mat{Y_i}$, $i\in\{1,~2,...,~n\}$.  
The coupled matrix-tensor factorization is given as the solution to the following optimization problem:

\begin{equation}
\displaystyle \min_{\mat{A_i},\mat{D_i}} \|\tensor{T} - \displaystyle {\sum_{k}  \mathbf{a_1}_k \circ \mathbf{a_2}_k \circ...\circ \mathbf{a_n}_k }\|_{F}^{2} +\sum_{i=1}^n\|\mat{Y_i}-\mat{A_i}\mat{D_i}^T\|_{F}^{2} %+...+\|\mat{Y_n}-\mat{A_n}\mat{D_n}^T\|_{F}^{2}
\label{eq:factorization}
\end{equation}

\noindent where $\mathbf{a_i}_k$ is the %$i^{th}$ dimension vector of the $f^{th}$ component of the PARAFAC decomposition of $\tensor{T}$ and forms the 
$k^{th}$ column of $\mat{A_i}$.  
The idea behind the coupled matrix-tensor decomposition is that we decompose $\tensor{T}$ and $\mat{Y_i}$ to latent factors that are coupled in the shared dimension.  
This joint factorization essentially provides a low dimensional embedding of the data in a common contextual subspace that can enable a variety of tasks including ranking.    



% you can have two matrices - one for the indices during the loses and one for the indices during the wins
